First measurement of neutron capture multiplicity in neutrino-oxygen neutral-current quasi-elastic-like interactions using an accelerator neutrino beam

We report the first measurement of neutron capture multiplicity in neutrino-oxygen neutral-current quasi-elastic-like interactions at the gadolinium-loaded Super-Kamiokande detector using the T2K neutrino beam, which has a peak energy of about 0.6 GeV. A total of 30 neutral-current quasi-elastic-like event candidates were selected from T2K data corresponding to an exposure of $1.76\times10^{20}$ protons on target. The $\gamma$ ray signals resulting from neutron captures were identified using a neural network. The flux-averaged mean neutron capture multiplicity was measured to be $1.37\pm0.33\text{ (stat.)}$$^{+0.17}_{-0.27}\text{ (syst.)}$, which is compatible within $2.3\,\sigma$ than predictions obtained using our nominal simulation. We discuss potential sources of systematic uncertainty in the prediction and demonstrate that a significant portion of this discrepancy arises from the modeling of hadron-nucleus interactions in the detector medium.

==> Tables/5_BonsaiVertex.tex <==
\begin{table}[htbp]
\centering
\caption{Non-positional reduction parameters uncertainties.}
\label{tab:NCQE_Bonsai}
\scalebox{0.8}{
\begin{tabular}{lll}
\hline
Reduction parameter & Description & Uncertainty \\
\hline
$E_{\text{rec}}$ & Reconstructed energy & $\pm 5 \%$ \\
OvaQ & Vertex and angular goodness coefficient & $\pm 1.5 \%$ \\
$\theta_C$ & Cherenkov angle & $\pm 2$ degree \\
\hline
\end{tabular}
}
\end{table}
